Deep Learning at 15PF: Supervised and Semi-Supervised Classification for Scientific Data

This paper presents the first, 15-PetaFLOP Deep Learning system for solving scientific pattern classification problems on contemporary HPC architectures. We develop supervised convolutional architectures for discriminating signals in high-energy physics data as well as semi-supervised architectures for localizing and classifying extreme weather in climate data. Our Intelcaffe-based implementation obtains $\sim$2TFLOP/s on a single Cori Phase-II Xeon-Phi node. We use a hybrid strategy employing synchronous node-groups, while using asynchronous communication across groups. We use this strategy to scale training of a single model to $\sim$9600 Xeon-Phi nodes; obtaining peak performance of 11.73-15.07 PFLOP/s and sustained performance of 11.41-13.27 PFLOP/s. At scale, our HEP architecture produces state-of-the-art classification accuracy on a dataset with 10M images, exceeding that achieved by selections on high-level physics-motivated features. Our semi-supervised architecture successfully extracts weather patterns in a 15TB climate dataset. Our results demonstrate that Deep Learning can be optimized and scaled effectively on many-core, HPC systems.

==> 11-references.tex <==
%\section{References}
%\textcolor{red}{1pg max}
\rem{(1 p max)}

\begin{thebibliography}{1}

% from http://inspirehep.net/record/1480037
\bibitem{ATLAS:2016nij} 
  The ATLAS collaboration [ATLAS Collaboration],
  ``Search for massive supersymmetric particles in multi-jet final states produced in pp collisions at $\sqrt{s}~=$~13 TeV using the ATLAS detector at the LHC,''
  ATLAS-CONF-2016-057.


\bibitem{HepNN}
C. Peterson, Nuclear Instruments and Methods A279 (1988) 537.


\bibitem{HepNN2}
 B. Denby, Computer Physics Communications 49 (1988) 429.

 
\bibitem{Delphes} 
  The DELPHES 3 collaboration, de Favereau, J., Delaere, C. et al. J. High Energ. Phys. (2014) 2014: 57. doi:10.1007/JHEP02(2014)057

\bibitem{Pythia} 
  T. Sjostrand, S. Mrenna and P. Skands, JHEP05 (2006) 026, Comput. Phys. Comm. 178 (2008) 852.

\bibitem{fastjet}
M. Cacciari, G.P. Salam and G. Soyez, Eur.Phys.J. C72 (2012) 1896 [arXiv:1111.6097]


\bibitem{jetimage1} L. de Oliveira, M. Kagan, L. Mackey, B. Nachman and A. Schwartzman, Jet-images - deep learning edition, JHEP 07 (2016) 069 [arXiv:1511.05190].
\bibitem{jetimage2}
P. T. Komiske, E. M. Metodiev and M. D. Schwartz, Deep learning in color: towards automated quark/gluon jet discrimination [arXiv:1612.01551].

\bibitem{CUDNNv5}
  ``NVIDIA cuDNN'', https://developer.nvidia.com/cudnn.

\bibitem{MKL2017DeepLearning}
  ``Introducing DNN primitives in Intel(R) Math Kernel Library'', https://software.intel.com/en-us/articles/introducing-dnn-primitives-in-intelr-mkl.

\bibitem{libxsmm}
A.~Heinecke, G.~Henry, M.~Hutchinson and H.~Pabst, ``LIBXSMM: Accelerating Small Matrix Multiplications by Runtime Code Generation'', SC 2016.

\bibitem{DeepBench}
DeepBench. https://github.com/baidu-research/DeepBench

\bibitem{Krizhevsky14}
A.~Krizhevsky, ``One weird trick for parallelizing convolutional neural networks'', https://arxiv.org/abs/1404.5997.

\bibitem{Dipankar16}
D.~Das, S.~Avancha et al., ``Distributed Deep Learning Using Synchronous Stochastic Gradient Descent'', https://arxiv.org/abs/1602.06709.

\bibitem{Firecaffe}
F.~N.~Iandola, K.~Ashraf, M.~W.~Moskewicz and K.~Keutzer, ``FireCaffe: near-linear acceleration of deep neural network training on compute clusters'', https://arxiv.org/abs/1511.00175.

\bibitem{intelcaffe}
Intel$\textsuperscript{\textregistered}$  distribution of Caffe*, https://github.com/intel/caffe

\bibitem{mlsl}
Intel$\textsuperscript{\textregistered}$ Machine Learning Scaling Library for Linux* OS, https://github.com/01org/MLSL 

\bibitem{eplib}
S. Sridharan, J. Dinan, and D. Kalamkar, ``Enabling efficient multithreaded MPI communication through a library-based implementation of MPI endpoints'', SC 2014.

\bibitem{winograd}
A.~Lavin and S.~Gray, ``Fast Algorithms for Convolutional Neural Networks'', https://arxiv.org/abs/1509.09308

\bibitem{courbariaux14}
M. Courbariaux, Y. Bengio and J.-P. David, ``Training deep neural networks with low precision multiplications'', https://arxiv.org/abs/1412.7024.

\bibitem{hubara16}
I. Hubara, M. Courbariaux, D. Soudry, R. El-Yaniv and Y. Bengio, 
``Quantized Neural Networks: Training Neural Networks with Low Precision Weights and Activations'', https://arxiv.org/abs/1609.07061.

\bibitem{gupta15}
S. Gupta, A. Agrawal, K. Gopalakrishnan, and P. Narayanan, ``Deep learning with limited numerical precision'', https://arxiv.org/abs/1502.02551.

\bibitem{gysel16}
P. Gysel, M. Motamedi, and S. Ghiasi, ``Hardware oriented
approximation of convolutional neural networks'', https://arxiv.org/abs/1604.03168.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% <IOANNIS>
\bibitem{hadjis2016omnivore}
Stefan Hadjis, Ce~Zhang, Ioannis Mitliagkas, Dan Iter, and Christopher R{\'e}.
\newblock Omnivore: An optimizer for multi-device deep learning on cpus and
  gpus.
\newblock {\em arXiv preprint arXiv:1606.04487}, 2016.

\bibitem{keskar2016large}
Nitish~Shirish Keskar, Dheevatsa Mudigere, Jorge Nocedal, Mikhail Smelyanskiy,
  and Ping Tak~Peter Tang.
\newblock On large-batch training for deep learning: Generalization gap and
  sharp minima.
\newblock {\em arXiv preprint arXiv:1609.04836}, 2016.

\bibitem{chen2016revisiting}
Jianmin Chen, Rajat Monga, Samy Bengio, and Rafal Jozefowicz.
\newblock Revisiting distributed synchronous sgd.
\newblock {\em arXiv preprint arXiv:1604.00981}, 2016.

\bibitem{tsitsiklis1986distributed}
John Tsitsiklis, Dimitri Bertsekas, and Michael Athans.
\newblock Distributed asynchronous deterministic and stochastic gradient
  optimization algorithms.
\newblock {\em IEEE transactions on automatic control}, 31(9):803--812, 1986.

\bibitem{recht2011hogwild}
Feng Niu, Benjamin Recht, Christopher Re, and Stephen Wright.
\newblock Hogwild: A lock-free approach to parallelizing stochastic gradient
  descent.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  693--701, 2011.

\bibitem{mania2015perturbed}
Horia Mania, Xinghao Pan, Dimitris Papailiopoulos, Benjamin Recht, Kannan
  Ramchandran, and Michael~I Jordan.
\newblock Perturbed iterate analysis for asynchronous stochastic optimization.
\newblock {\em arXiv preprint arXiv:1507.06970}, 2015.

\bibitem{chaturapruek2015asynchronous}
Sorathan Chaturapruek, John~C Duchi, and Christopher R{\'e}.
\newblock Asynchronous stochastic convex optimization: the noise is in the
  noise and sgd don't care.
\newblock In {\em NIPS}, pages 1531--1539, 2015.

\bibitem{de2015taming}
Christopher~M De~Sa, Ce~Zhang, Kunle Olukotun, and Christopher R{\'e}.
\newblock Taming the wild: A unified analysis of hogwild-style algorithms.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  2674--2682, 2015.

\bibitem{dean2012large}
Jeffrey Dean, Greg Corrado, Rajat Monga, Kai Chen, Matthieu Devin, Mark Mao,
  Andrew Senior, Paul Tucker, Ke~Yang, Quoc~V Le, et~al.
\newblock Large scale distributed deep networks.
\newblock In {\em Advances in neural information processing systems}, pages
  1223--1231, 2012.

\bibitem{chilimbi2014project}
Trishul Chilimbi, Yutaka Suzue, Johnson Apacible, and Karthik Kalyanaraman.
\newblock Project adam: Building an efficient and scalable deep learning
  training system.
\newblock In {\em 11th USENIX Symposium on Operating Systems Design and
  Implementation (OSDI 14)}, pages 571--582, 2014.

\bibitem{mitliagkas2016asynchrony}
Ioannis Mitliagkas, Ce~Zhang, Stefan Hadjis, and Christopher R{\'e}.
\newblock Asynchrony begets momentum, with an application to deep learning.
\newblock {\em arXiv preprint arXiv:1605.09774}, 2016.

\bibitem{DBLP:journals/pvldb/ZhangR14}
Ce~Zhang and Christopher Re.
\newblock Dimmwitted: {A} study of main-memory statistical analytics.
\newblock {\em {PVLDB}}, 7(12):1283--1294, 2014.

\bibitem{yunjie:abda16}
Liu, Yunjie, et al. 
\newblock "Application of Deep Convolutional Neural Networks for Detecting Extreme Weather in Climate Datasets." 
\newblock arXiv preprint arXiv:1605.01156, 2016.

@article{racah2016semi,
  title={Semi-Supervised Detection of Extreme Weather Events in Large Climate Datasets},
  author={Racah, Evan and Beckham, Christopher and Maharaj, Tegan and Pal, Christopher and others},
  journal={arXiv preprint arXiv:1612.02095},
  year={2016}
}
@inproceedings{redmon2016you,
  title={You only look once: Unified, real-time object detection},
  author={Redmon, Joseph and Divvala, Santosh and Girshick, Ross and Farhadi, Ali},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={779--788},
  year={2016}
}
@inproceedings{liu2016ssd,
  title={SSD: Single shot multibox detector},
  author={Liu, Wei and Anguelov, Dragomir and Erhan, Dumitru and Szegedy, Christian and Reed, Scott and Fu, Cheng-Yang and Berg, Alexander C},
  booktitle={European Conference on Computer Vision},
  pages={21--37},
  year={2016},
  organization={Springer}
}
@inproceedings{ren2015faster,
  title={Faster r-cnn: Towards real-time object detection with region proposal networks},
  author={Ren, Shaoqing and He, Kaiming and Girshick, Ross and Sun, Jian},
  booktitle={Advances in neural information processing systems},
  pages={91--99},
  year={2015}
}

%%%%%%%% </IOANNIS>
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% </THORSTEN>
\bibitem{krizhevsky2012imagenet}
Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E
\newblock "Imagenet classification with deep convolutional neural networks."
\newblock {\em Advances in neural information processing systems}, pages 1097--1105, 2012

\bibitem{hahnloser2000digital}
Hahnloser, Richard HR and Sarpeshkar, Rahul and Mahowald, Misha A and Douglas, Rodney J and Seung, H Sebastian
\newblock "Digital selection and analogue amplification coexist in a cortex-inspired silicon circuit."
\newblock {\em Nature}, volume 405, number 6789, pages 947--951, 2000

\bibitem{he2015delving}
He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian
\newblock "Delving deep into rectifiers: Surpassing human-level performance on imagenet classification."
\newblock {\em Proceedings of the IEEE international conference on computer vision}, pages 1026--1034, 2015

\bibitem{kingma2014adam}
Kingma, Diederik and Ba, Jimmy
\newblock "Adam: A method for stochastic optimization."
\newblock {\em arXiv preprint arXiv:1412.6980}, 2014
%%%%%%%% </THORSTEN>
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{thebibliography}

